Keep It Private: Unsupervised Privatization of Online Text

Authorship obfuscation techniques hold the promise of helping people protect their privacy in online communications by automatically rewriting text to hide the identity of the original author. However, obfuscation has been evaluated in narrow settings in the NLP literature and has primarily been addressed with superficial edit operations that can lead to unnatural outputs. In this work, we introduce an automatic text privatization framework that fine-tunes a large language model via reinforcement learning to produce rewrites that balance soundness, sense, and privacy. We evaluate it extensively on a large-scale test set of English Reddit posts by 68k authors composed of short-medium length texts. We study how the performance changes among evaluative conditions including authorial profile length and authorship detection strategy. Our method maintains high text quality according to both automated metrics and human evaluation, and successfully evades several automated authorship attacks.

==> tables/comment_scale.tex <==


\begin{table*}[ht]
\caption{Verification performance (measured with F1 using a CNG-classifier) across increasing number of comments for \texttt{REDDIT}}
  \label{tab:verification_comment_scale}
\begin{tabularx}{.5\textwidth}{llrrrrrrrr}
    
% {@{}llrrrrrrrrr@{}} % repeats {c|} 18 times
\toprule
 % &  & \multicolumn{3}{c}{2,4,8,12,16 comments }  \\ 
 
  Model & \textit{FT?} & 2 & 4 & 8 & 12 & 16 \\  
  \hline\hline
  No-op & \textit{-} & 0.02 & 0.144 & 0.55 & 0.862 & 0.919 \\
  Normalizer & \textit{-} & 0.02 & 0.144 & 0.55 & 0.862 & 0.919 \\
Backtranslator & \textit{-} & 0.02 & 0.125 & 0.523 & 0.84 & 0.927\\\hline
\multirow{2}{*}{KiP-T5} & Base & 0.02 & 0.104 & 0.68 & 0.906 & 0.958 \\
& Para & 0.02 & 0.086 & 0.445 & 0.799 & 0.917 \\\hline
\multirow{2}{*}{KiP-BART} & Base & 0.02 & 0.103 & 0.605 & 0.898 & 0.946\\
& Para & 0.02 & 0.113 & 0.466 & 0.814 & 0.936 \\\hline

\bottomrule
\end{tabularx}


\end{table*}



==> tables/comment_scale2.tex <==


\begin{table*}[ht]

\begin{tabularx}{.5\textwidth}{llrrrrrrrr}
    
% {@{}llrrrrrrrrr@{}} % repeats {c|} 18 times
\toprule
 % &  & \multicolumn{3}{c}{2,4,8,12,16 comments }  \\ 
 
  Model & \textit{FT?} & 1 & 4 & 8 & 16 & 32 \\  
  \hline\hline
  No-op & \textit{-} & 1 & 1 & 1 & 0.84 & 0.226 \\
  Normalizer & \textit{-} & 0.69 & 0.784 & 0.862 & 0.832 & 0.24 \\
  Stylo & \textit{-} & 0.706 & 0.748 & 0.851 & 0.766 & 0.159 \\
Backtranslator & \textit{-} & 0.677 & 0.757 & 0.859 & 0.798 & 0.221\\\hline
KiP-GPT2 & \textit{-} & 0.71 & 0.777 & 0.823 & 0.748 & 0.151\\\hline
\multirow{2}{*}{KiP-T5} & Base & 0.763 & 0.856 & 0.92 & 0.896 & 0.234 \\
& Para & 0.684 & 0.752 & 0.838 & 0.748 & 0.148 \\\hline
\multirow{2}{*}{KiP-BART} & Base & 0.719 & 0.806 & 0.872 & 0.869 & 0.226\\
& Para & 0.654 & 0.752 & 0.838 & 0.782 & 0.187 \\\hline

\bottomrule
\end{tabularx}
\caption{Verification performance (measured with F1 using a CNG-classifier) across increasing number of comments (1,4,8,16,32) for \texttt{REDDIT}. }
  \label{tab:verification_comment_scale2}

\end{table*}



==> tables/human_eval.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|}
        & No paraphrase & Ungrammatical paraphrase & Grammatical paraphrase \\\hline
        Round-trip MT & 22.22\% & 23.90\% & 53.87\% \\
        \hline
        Stylo & 20.54\% & 44.11\% & 35.35\%  \\
        \hline
        KiP-BART-para & 29.96\% & 28.95\% & 41.08\% \\
        \hline
    \end{tabular}
    \caption{Human Evaluation results}
    \label{tab:human_eval}
\end{table}

==> tables/pan_results.tex <==

% \begin{table*}
% \begin{tabular}{llrrrrrrrrr}  % repeats {c|} 18 times
% \toprule
%  &  & \multicolumn{3}{c}{L1} & \multicolumn{3}{c}{L2} & \multicolumn{3}{c}{L3}  \\ 
%   Models & \textit{k} & BLEU & SARI & ARI  & BLEU & SARI & ARI & BLEU & SARI & ARI\\  
%   \midrule
% CCMT-Supervised  & - & 18.16 & 0.51 & 11.83 & 24.35 & 0.466 & 10.15 & 29.76 & 0.412 & 8.05 \\
%  \addlinespace[0.2cm]

% \multirow{4}{*}{Joint} & 0 & 19.24 & 0.09 & 12.71 & 27.24 & 0.12 & 12.71 & 34.82 & 0.14 & 12.48 \\
% % \cline{2-11}
% & 1 & 19.17 & 0.33 & 12.64 & 27.22 & 0.34 & 12.75 & \textbf{35.28} & 0.34 & 12.60 \\
% % \cline{2-11}
% & 4 & 19.25 & 0.32 & 12.74  & 27.08  & 0.335  & 12.66 & 35.09 & 0.33 & 12.66 \\
% % \cline{2-11}
% & 8 & \textbf{19.68} & 0.33 & 12.65 & 27.23  & 0.339 & 12.60 & 35.22 & 0.33 & 12.58 \\ 

%  \addlinespace[0.2cm]

% \multirow{4}{*}{Pipeline (T -> S)} & 0 & 18.65 & 0.39 & 12.12 & 20.34 & 0.247 & 12.12 & \textbf{24.13} & 0.41 & 12.12 \\
% % \cline{2-11}
% & 1 & 19.62 & 0.38  & 13.08 & \textbf{23.94} & 0.407 & 12.96 & 21.58 & 0.401 & 11.53 \\ 
% % \cline{2-11}
% & 4 & \textbf{19.73} & 0.39 & 12.66 & 23.64 & 0.417 & 11.547 & 20.16 & 0.39 & 10.28\\
% % \cline{2-11}
% & 8 & 19.35 & 0.38 & 12.83 & 21.43 & 0.403 & 11.327 & 21.39 & 0.40 & 10.09\\
% \bottomrule

% \end{tabular}
%     \caption{Simplification metrics for outputs, produced by models conditioned on \textit{k} leveled exemplars, a task-specific prompt, and the input text. The pipeline approach varies settings for simplification. It first translates the source using only a translation prompt and then simplifies the translation by demonstrating with exemplars and providing a simplification-specific prompt.}
%     \label{tab:resultsTable}
% \end{table*}




\begin{table*}[ht]
\centering
\begin{tabularx}{\textwidth}{ll|rrrr|r|rrrr}
% {@{}llrrrrrrrrr@{}} % repeats {c|} 18 times
\toprule
% & & \multicolumn{6}{c}{\texttt{PAN}} \\
 &  & \multicolumn{4}{c|}{Privacy} & \multicolumn{1}{c|}{Sense} & \multicolumn{2}{c}{Soundness}  \\ 
  Systems & \textit{FT} & LUAR ↑ & R@8 ↓ & MRR ↓ & CNG-F1 ↓ & SBERT ↑ & COLA-diff & COLA-out \\  
  \hline\hline
Normalizer & - & 0.124 & 0.18 & 0.15  & 0.998 & \textbf{0.998} & 0.85 & 0.767 \\  
Heuristic Search & - & - & - & -  & - & - & - & - \\  
BT (en-de) & - & 0.143 & 0.13 & 0.05 & 0.612 & 0.938 & 0.879 & 0.86 \\  \hline
KiP-GPT2 & - & 0.165 & \textbf{0.02} & \textbf{0.0} & 0.849 & 0.904 & 0.73 & 0.66 \\  \hline
% KiP & GPT2 & 0 & 0 & 0  & 0 & 0 & 0 & 0 \\  
\multirow{2}{*}{KiP-T5} & Base & \textbf{0.27} & 0.08 & 0.07  & \textbf{0.0} & 0.46 & 0.638 & 0.676 \\  
& Para & 0.151 & 0.15 & 0.15  & 0.383 & 0.723 & 0.763 & 0.821 \\  \hline

\multirow{2}{*}{KiP-BART} & Base & 0.177 & 0.14 & 0.12  & 0.9 & 0.71 & 0.621 & 0.599 \\  
& Para & 0.142 & 0.04 & 0.02  & 0.084 & 0.909 & 0.784 & 0.735 \\  
\bottomrule
\end{tabularx}
    \caption{Evaluation for the \texttt{FANFIC} dataset across models. This table shows a controlled ablation of the base generator, and compares their performance to existing baselines. [TODO: cover same models as in reddit, investigate why these results seem so unstable.]}
    \label{tab:panResults}
\end{table*}


==> tables/paraphrasing_edits.tex <==


\begin{table*}[ht]

\begin{tabularx}{.5\textwidth}{llrrr}
    
% {@{}llrrrrrrrrr@{}} % repeats {c|} 18 times
\toprule
 &  & \multicolumn{3}{c}{Levenshtein edits }  \\ 
 
  Setting & \textit{EC?} & DEL & REP & ADD \\  
  \hline\hline
\multirow{2}{*}{Attribution} & Yes & - & - & - \\
& No & - & - & -  \\\hline
\multirow{2}{*}{Verification} & Yes & - & - & - \\
& No & - & - & -  \\\hline
\bottomrule
\end{tabularx}
\caption{Levenshtein edits made by \texttt{KiP-BART-Para}. In the attribution setting, ``Evaded Capture?'' (EC?) are on needle author profiles created by concatenating 8 comments that had did not successfully retrieve the author in a top-8 list. In the verification setting, EC? is the prediction of ``different authors'' on same-author pairs.}
  \label{tab:paraphrasing_edits}

\end{table*}



==> tables/reward_ablation.tex <==
\usepackage{caption}
\captionsetup{width=.75\textwidth}
\begin{table*}[p]
\centering
\begin{tabularx}{0.65\textwidth}{l @{\makebox[1.5em][r]{\rownumber\space}} | llrrrr}
    
% {@{}llrrrrrrrrr@{}} % repeats {c|} 18 times
\toprule

  \multicolumn{1}{l}{Base} & \multicolumn{1}{l}{\textit{weights}} & \multicolumn{1}{l}{LUAR} & \multicolumn{1}{l}{SBERT} & \multicolumn{1}{r}{CoLa} \\  
  \hline\hline
\multirow{4}{*}{\texttt{GPT2}} & $\gamma_1=\textbf{4},\gamma_2=3,\gamma_3=2$ & \textbf{0.6187} & 0.518 & 0.817\\
& $\gamma_1=\textbf{4},\gamma_2=3,\gamma_3=\textbf{4}$ & 0.417 & 0.8 & 0.66 \\
& $\gamma_1=0,\gamma_2=2,\gamma_3=\textbf{5}$ & 0.527 & 0.621 & 0.881 \\
& $\gamma_1=2,\gamma_2=2,\gamma_3=2$ & 0.562 & \textbf{0.624} & \textbf{0.895} \\
\hline
\multirow{2}{*}{\texttt{BART-p}} & $\gamma_1=\textbf{4},\gamma_2=3,\gamma_3=2$ & \textbf{0.429} & 0.717 & 0.555 \\
& $\gamma_1=\textbf{4},\gamma_2=3,\gamma_3=\textbf{4}$ & 0.36 & 0.829 & 0.537 \\
& $\gamma_1=2,\gamma_2=2,\gamma_3=\textbf{5}$ & 0.295 & \textbf{0.88} & \textbf{0.719} \\
& $\gamma_1=2,\gamma_2=2,\gamma_3=2$ & 0.296 & 0.875 & 0.7047 \\

\hline
\bottomrule
 \end{tabularx}\caption{Impact of varying weights for privacy: $\gamma_1,\gamma_2$ and meaning preservation: $\gamma_3$ in \autoref{combined_reward} during training for two base generators using KiP. The highest values associated with the $\gamma_i$ are bolded to emphasize which component had larger impacts on $R_S$.}
  \label{tab:reward_ablation}


\end{table*}



